Looking Beyond Sentence-Level Natural Language Inference for Downstream Tasks

In recent years, the Natural Language Inference (NLI) task has garnered significant attention, with new datasets and models achieving near human-level performance on it. However, the full promise of NLI -- particularly that it learns knowledge that should be generalizable to other downstream NLP tasks -- has not been realized. In this paper, we study this unfulfilled promise from the lens of two downstream tasks: question answering (QA), and text summarization. We conjecture that a key difference between the NLI datasets and these downstream tasks concerns the length of the premise; and that creating new long premise NLI datasets out of existing QA datasets is a promising avenue for training a truly generalizable NLI model. We validate our conjecture by showing competitive results on the task of QA and obtaining the best reported results on the task of Checking Factual Correctness of Summaries.

==> discards/CFCS.tex <==


Having validated the long-premise conjecture, we show the utility of long-premise NLI datasets by using them to solve the task of checking factual consistencies of summaries (CFCS).
% \sout{
% For this, we first obtain our entailment scorer by fine-tuning multiple choice classification model (Figure \ref{fig:model_mc}) on the NLI form RACE dataset and then perform the task of  CFCS (zero-shot). \sout{by using it as a two class entailment model (as described in Section \ref{sec:transferable_modeling}).} 
% }
We setup the task in two forms: (1) as a classification task; (2) as a ranking task. Both these forms are targeted towards picking a factually correct summary from several machine generated summaries.

\subsubsection{CFCS as classification}
\label{subsubsec:results_cfcs_classification}
In this form, given a document and a corresponding summary sentence, the model needs to identify if the sentence is factually correct w.r.t to document (is entailed) or not. 
%We use the dev and test dataset provided by \citet{kryscinski2019evaluating} for this task. 
In order to perform the classification, we first obtain our entailment scorer by fine-tuning multiple choice classification model (Figure \ref{fig:model_mc}) on the NLI form of the RACE dataset and use the dev set\footnote{\label{fn:factcc}We use the dev and test dataset provided by \citet{kryscinski2019evaluating} for this task.} to calibrate a threshold as described in section \ref{sec:transferable_modeling} to obtain the two-class entailment model (Figure \ref{fig:model_entailment}). The results of using this model on the test set\textsuperscript{\footnotemark[\ref{fn:factcc}]} are given in Table \ref{tab:results-factcc}. As seen, the model trained on the NLI form of the RACE dataset (RACE\textsubscript{Hybrid}) outperforms the baselines as well as the model trained on MultiNLI.

\begin{table}[!ht]
\centering
\begin{threeparttable}

\begin{tabular}{@{}l|c|c@{}}
\toprule
    \textbf{Model} 
    & \begin{tabular}[c]{@{}c@{}}\textbf{Balanced}\\ \textbf{Accuracy }\end{tabular} 
    & \textbf{F1-score} \\ 
\midrule
    BERT+MultiNLI\tnote{\textasteriskcentered}   
        & 51.51 
        & 0.09\\
    FactCC\tnote{\textasteriskcentered}
        & 74.15 
        & 0.51\\
    FactCCX\tnote{\textasteriskcentered}
        & 72.88 
        & 0.50\\
    RoBERTa 
        & 49.89
        & 0.46 \\
    RoBERTa+MultiNLI 
        & 50.00
        & 0.47 \\
    % RoBERTa+RACE\textsubscript{Neural} 
    %     & \textbf{87.58}
    %     & \textbf{0.87}\\ 
    RoBERTa+RACE\textsubscript{Hyrbid} 
        & 82.99
        & 0.82\\ 
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
    \footnotesize
    \item [\textasteriskcentered] Taken from~\citet{kryscinski2019evaluating}
\end{tablenotes}
\vspace{-5pt}
\caption{Balanced accuracy on FactCC dataset.}
\label{tab:results-factcc}
\end{threeparttable}
\end{table}





\subsubsection{CFCS as ranking}

%\noindent(2) Further, we also use the dataset provided by \cite{Falke2019}, to setup the task as a ranking task, 

In this form, given a source document and a set of five\footnote{A variable number of these five machine generated summaries can be factually correct. However, there is always at least one incorrect summary in this set.} machine generated summaries, the model is required to rank at least one factually correct summary above all incorrect summary alternatives. 
We also solve the auxiliary task of sentence-pair ranking, where the premise document $D=\{d_1, d_2, \dots\}$ as well as the summary $S=\{s_1, s_2, \dots\}$ are divided into individual sentences and the model is required to decide if $d_i$ entails $s_j$ or not. 




\begin{table}[!ht]
\centering
\begin{threeparttable}
\begin{tabular}{@{}ll@{}}
\toprule
    \multicolumn{2}{c}{\textbf{Sentence-pair ranking task}} \\ 
    \midrule
        \textbf{Model}
        & \textbf{\% Corr. ($\uparrow$)} \\ 
    \midrule
        BERT+MultiNLI \tnote{*} 
            & 64.10\% \\
        FactCC\tnote{\textdagger}
            & 70.00\% \\
        QAGS\tnote{\ddag}
            & 72.10\% \\
        RoBERTa 
            & 56.03\% \\
        RoBERTa+MultiNLI 
            & 81.76\% \\
        % RoBERTa+RACE\textsubscript{Neural} 
        %     & \textbf{86.59\%} \\
        RoBERTa+RACE\textsubscript{Hybrid} 
            & \textbf{86.59\%} \\ 
\midrule
    \multicolumn{2}{c}{\textbf{Summary re-ranking task}\sout{\tnote{\mp}}}                         \\ 
    \midrule
        \textbf{Model}
            & \textbf{\% Corr. ($\uparrow$)} \\
        \midrule
        Original/unranked
            & 57.90\% \\
        ESIM*
            & 60.70\% \\
        RoBERTa 
            & 50.47\% \\
        RoBERTa+MultiNLI 
            & 49.53\% \\
        % RoBERTa+RACE\textsubscript{Neural} 
        %     & 73.83\% \\
        RoBERTa+RACE\textsubscript{Hybrid} 
            & \textbf{75.70}\% \\
\bottomrule
\end{tabular}%
\begin{tablenotes}[flushleft]
\footnotesize
    %\item [\mp] Uses the validation dataset as the test dataset is not available
    \item [*] Taken from~\citet{Falke2019}
    \item [\textdagger] Taken from~\citet{kryscinski2019evaluating}
    \item [\ddag] Taken from~\citet{wang2020asking}
\end{tablenotes}
\vspace{-5pt}
\caption{Fraction of examples where a factually correct summary takes the first rank. 
RACE\textsubscript{Hybrid} refers to the converted RACE datasets. \comment{I feel that we need a MNLI piecewise baseline (where we use aggregation on premise) because RoBERTa+MNLI is below ESIM which will raise questions. Their ESIM is using piecewise aggregation.}}
\label{tab:results-summary_ranking}
\end{threeparttable}
\end{table}

%As shown in Table \ref{tab:results-factcc} and Table \ref{tab:results-summary_ranking}, the models trained on the NLI for of the RACE dataset outperform the baselines as well as the model trained on MultiNLI. \sout{For the summary correctness dataset, we also show the results from \citet{wang2020asking} who attempt to solve the task by reducing it to the task of QA. We show that reduction to NLI is more helpful.} 
%\sout{
%Our converted dataset not only helps the model perform better than the MultiNLI model, but we achieve new state-of-the-art results on these tasks.
%To ascertain the cause of the poor performance of the model trained on MultiNLI, we also solve the task of sentence-pair ranking, where the premise (document) as well as the summary is divided into individual sentences and the model is asked to solve a sentence-level NLI task. As shown in Table \ref{tab:results-summary_ranking},
%}
Table \ref{tab:results-summary_ranking} shows that model trained on the NLI form of RACE outperforms all the baselines as well as the model trained on MultiNLI. It is particularly interesting to note that the model trained on MultiNLI is good at the task of sentence-pair  ranking but is unable to translate this to the task of summary re-ranking which has long premises.
% \newlyadded{It is useful to note that on the model trained on MultiNLI does reasonably well is the task of sentence-ranking where the average premise length is 25 words (Table \ref{tab:premise_lengths}).} 

These state-of-the-art results \comment{do we want to claim SOTA?} on both the forms of CFCS task further reinforce our long premise conjecture: models which learn entailment relationships from long premises perform much better at downstream tasks. 
% {This makes the converted datasets more suitable for downstream applications such as checking factual correctness in summaries and multiple choice reading comprehension where the premise is naturally very long. \comment{Do we want to add the premise length graph for CFCS here?}



%\newlyadded{Table \ref{tab:results-factcc} shows the results of models on FactCC. We show that the model trained on the neural-conversion data outperforms all other models.}


% \begin{table}[!ht]
% \centering
% \begin{threeparttable}
% \begin{tabular}{@{}lcc@{}}
% \toprule
% \textbf{\textbf{Model}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}\textbf{Balanced} \\\textbf{Accuracy}\end{tabular}} &
%   \textbf{\textbf{F1}} \\ \midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}BERT + MNLI\tnote{*}\end{tabular}}     & \multicolumn{1}{c}{51.51} & 8.82 \\\midrule
% \multicolumn{1}{l}{FactCC \tnote{*}}                                                     & \multicolumn{1}{c}{74.15} & 51.06 \\\midrule
% \multicolumn{1}{l}{FactCCX \tnote{*}}                                                    & \multicolumn{1}{c}{72.88} & 50.05 \\ \midrule
% %\multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}RoBERTa + RACE\_QA\end{tabular}} & \multicolumn{1}{c}{80.57} & 80.35 \\\midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}RoBERTa + RACE\_NLI \\ (Neural conversion)\end{tabular}} &
%   \multicolumn{1}{c}{\textbf{87.58}} &
%   \textbf{86.57} \\\midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}RoBERTa + MNLI\end{tabular}}   & \multicolumn{1}{c}{50}    & -      \\ \bottomrule
% \end{tabular}
% \caption{Results on FactCC. Results using BERT MNLI, FactCC and FactCCX are from \citet{kryscinski2019evaluating}}
% \label{tab:results-factcc}
% \begin{tablenotes}
% \end{tablenotes}
% \end{threeparttable}
% \end{table}



%\begin{table*}[]
%    \centering
%    \begin{tabular}{l|c|c}
%    \toprule
%        \textbf{Model} & \textbf{Balanced Accuracy } & \textbf{F1-score} \\
%    \bottomrule
%        BERT+MNLI* & 51.51 & 0.0882  \\
%        FactCC* & 74.15 & 0.5106 \\
%        FactCCX* & 72.88 & 0.5005 \\
%        % RoBERTa+RACE-QA & 80.57 & 0.8035 \\
%        RoBERTa+MNLI & 50 & -\\
%        RoBERTa+RACE\textsubscript{Neural} & \textbf{87.58} & \textbf{0.8657} \\
%    \bottomrule
%    \end{tabular}
%    \caption{Results on FactCC. Results using BERT MNLI, FactCC and FactCCX are from \citet{kryscinski2019evaluating}. RACE\textsubscript{Neural} refers to the converted RACE dataset created 
%using the BART model.}
%    \label{tab:results-factcc}
%\end{table*}





%%%%%%%%%% split tables %%%%%%%%
% using combined table above
%\begin{table}[!ht]
%\centering
%\begin{tabular}{l|c}
%\toprule
%    \textbf{Model} & \textbf{\% Correct ($\uparrow$)} \\
%\bottomrule
%    BERT NLI*        & 64.1\%  \\ %\midrule
%    FactCC*          & 70.0\%  \\ %\midrule
%    QAGS*            & 72.1\%  \\ %\midrule
%    % RoBERTa+RACE\_QA & 83.64\% \\ \midrule
%    RoBERTa+MNLI & 81.76\% \\ %\midrule
%    RoBERTa+RACE\textsubscript{Neural} &  \textbf{86.59\%} \\ \bottomrule
%\end{tabular}
%\caption{Results on the sentence-pair ranking task from \cite{falke2019ranking}. Results using BERT NLI is from \citet{falke2019ranking}; FactCC is from \citet{kryscinski2019evaluating}; QAGS is from \citet{wang2020asking}. RACE\textsubscript{Neural} refers to the converted RACE dataset created 
%using the BART model.}
%\label{tab:results-summary_ranking}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|l|c}
%\toprule
%\textbf{Split} &
%\textbf{Model} &
%  \textbf{\% Corr. ($\uparrow$)} \\ %\midrule
%  \bottomrule
%    \multirow{4}{*}{Val} 
%        & Original*        & 57.9\%  \\ %\midrule
%        & ESIM*          & 60.7\%  \\ %\midrule
%        % RoBERTa+RACE\_QA & 83.64\% \\ \midrule
%        & RoBERTa+MNLI & 77.12\% \\ %\midrule
%        & RoBERTa+RACE\textsubscript{Neural} &  \textbf{92.25\%} \\ \midrule
%    \multirow{4}{*}{Test} 
%        & Original*        & 74\%  \\ %\midrule
%        & ESIM*          & 71\%  \\ %\midrule
%        & RoBERTa+MNLI & 75\% \\ %\midrule
%        & RoBERTa+RACE\textsubscript{Neural} &  \textbf{91.66\%} \\ %\midrule
%\bottomrule
%\end{tabular}
%\caption{Results on the summary reranking task from \cite{falke2019ranking}. Orignal results and those using ESIM are from \citet{falke2019ranking}. RACE\textsubscript{Neural} refers to the converted RACE dataset created 
%using the BART model.}
%\label{tab:results-summary_ranking}
%\end{table}

%\begin{table*}[]
%    \centering
%    \begin{tabular}{l|c|c}
%    \toprule
%        \textbf{Model} & \textbf{Num Labels} & \textbf{\% Correct ($\uparrow$)} \\
%    \bottomrule
%        BERT NLI* & 3 & 64.1\% \\
%        FactCC* & 3 & 70.0\% \\
%        QAGS* & 3 & 72.1\% \\
%    \hline
%        RoBERTa+RACE-QA & 2 & 83.64\% \\
%        RoBERTa+RACE-NLI (Neural) & 2 & \textbf{86.59\%} \\
%        RoBERTa+MNLI & 2 & 81.76\% \\
%    \bottomrule
%    \end{tabular}
%    \caption{\newlyadded{Results on the summary correctness dataset from \cite{falke2019ranking}. Numbers for BERT NLI, FactCC and QAGS as reported by \cite{wang2020asking}}}
%    \label{tab:results-summary_ranking}
%\end{table*}



==> discards/Fragments_misc.tex <==


We inspect the models trained on the converted dataset to understand if they capture sentence-level semantics. We use the systematically generated datasets developed by \citet{richardson2019probing} to probe NLI datasets and models for a variety of semantic phenomenon. We first finetune RoBERTa in the multiple choice setting (Figure \ref{fig:model_mc}) on RACE\textsubscript{Neural} and RACE\textsubscript{Hybrid}. Subsequently, we transfer the model to the two class entailment setting (Figure \ref{fig:model_entailment}) to perform zero-shot evaluation on the semantic fragment benchmark as described in Section \ref{sec:transferable_modeling}.


{Tables \ref{tab:utility_nli-semantic_fragments} 
% and \ref{tab:utility_nli-dnc} 
shows the performance of the models on the different semantic phenomena. We show that the converted NLI datasets are broadly at par with MNLI in terms of capturing sentence-level semantic phenomena. The ease of creation of these converted datasets can facilitate the development of diverse NLI datasets and subsequently allow NLI to act as an abstraction layer for various different natural language processing tasks.}


\begin{table*}[!ht]
\centering
% \resizebox{0.48\textwidth}{!}{%
\begin{tabular}{
    l|
    c|
    c|
    c}
\toprule
% \textbf{\begin{tabular}[c]{@{}l@{}}\textbf{Semantic}\\  \textbf{Fragment}\end{tabular}} 
    \textbf{Semantic Fragment}
    % & \textbf{RACE-QA} 
    & \textbf{RACE\textsubscript{Hybrid}}
    & \textbf{RACE\textsubscript{Neural}} 
    & \textbf{MNLI} \\ %\midrule
\midrule
Boolean
    % & \multicolumn{1}{c}{75.5} 
    & 84.00
    & 86.50
    & \textbf{93.00} \\ %\midrule
Comparative
    % & \multicolumn{1}{c}{55.8} 
    & 66.80
    & 62.20
    & \textbf{74.50} \\ %\midrule
Conditional
    % & \multicolumn{1}{c}{\textbf{83.4}} 
    & \textbf{83.40}
    & \textbf{83.40}
    & 61.10 \\ %\midrule
Counting
    % & \multicolumn{1}{c}{54.3} 
    & 45.30
    & \textbf{62.30}
    & 54.00 \\ %\midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Monotonicity\\ (Hard)\end{tabular}} 
Monotonicity (Hard)
    % & \multicolumn{1}{c}{44.2} 
    & 50.90
    & 50.70
    & \textbf{62.80} \\ %\midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Monotonicity \\ (Simple)\end{tabular}}
Monotonicity (Simple)
    % & \multicolumn{1}{c}{61.8} 
    & \textbf{67.60}
    & \textbf{67.60}
    & 62.00 \\ %\midrule
Negation
    % & \multicolumn{1}{c}{70.7} 
    & 86.80
    & \textbf{89.60}
    & 82.50 \\ %\midrule
Quantifier
    % & \multicolumn{1}{c}{56.0} 
    & 71.00
    & 75.70
    & \textbf{77.60} \\ \midrule
\textbf{Overall}
    % & \multicolumn{1}{c}{62.7} 
    & 69.48
    & \textbf{72.25}
    & 70.94 \\ \bottomrule
\end{tabular}%
% }
\caption{Results on the Semantic Fragments dataset from \cite{richardson2019probing}. RACE\textsubscript{Neural} and RACE\textsubscript{Hybrid} refer to the converted RACE datasets.}
\label{tab:utility_nli-semantic_fragments}
\end{table*}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{
%         l|
%         % c|
%         % c|
%         c|
%         c}
%     \toprule
%         \textbf{Sem. Phenomenon} 
%             % & \textbf{\% of Data} 
%             % & RACE-QA 
%             & \textbf{RACE\textsubscript{Neural}}
%             & \textbf{MNLI} \\
%     \midrule
%         Factuality 
%             % & 7.29\% 
%             % & 61.38 
%             & 61.47 
%             & \textbf{67.39} \\
%         NER 
%             % & 63.18\% 
%             % & \textbf{73.19} 
%             & \textbf{69.28} 
%             & 58.36 \\
%         Pun 
%             % & 2.94\% 
%             % & 50 
%             & 49.71 
%             & \textbf{58.54} \\
%         Sentiment 
%             % & 1.01\% 
%             % & 93.83 
%             & \textbf{94.17} 
%             & 68.5 \\
%         Lexicosyntactic (MV) 
%             % & 1.98\% 
%             % & 36.72 
%             & 35.62 
%             & \textbf{43.49} \\
%         Lexicosyntactic (VN) 
%             % & 0.27\% 
%             % & 46.88 
%             & 48.13 
%             & \textbf{55} \\
%         Lexicosyntactic (VC) 
%             % & 23.32\% 
%             % & \textbf{51.73} 
%             & \textbf{50.25} 
%             & 46.59 \\
%     \midrule
%         \textbf{Overall} 
%             % & 100\% 
%             % & \textbf{66.06} 
%             & \textbf{63.22} 
%             & 56.08 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Results on the Diverse Natural Language Inference dataset from \cite{poliak2018collecting}. RACE\textsubscript{Neural} refers to the converted RACE dataset created using the BART model. MV refers to the MegaVeridicality dataset; VN to the VerbNet dataset; VC to the VerbCorner dataset. \comment{Anshuman: Lets drop this result}}
%     \label{tab:utility_nli-dnc}
% \end{table}

==> discards/long_premise_conjecture.tex <==
%%%%%%%%%%%%%%%%%%% EXP %%%%%%%%%%%%%%%%%%%


%\sout{For the purpose of evaluating the utility of our converted datasets, we choose the tasks MCRC and CFCS, as mentioned in Section \ref{sec:nli_for_downstream}. We first train our transferable RoBERTa-based model on the converted RACE dataset in NLI format. We then test the transferability of this model by performing zero-shot evaluations on the other converted MCRC datasets. We perform similar zero-shot evaluations by using a model trained on MultiNLI instead. Table \ref{tab:results_mcrc} shows the performance of these models on each of the converted MCRC datasets. We can clearly see that the performance of the models trained on the converted MCRC datasets beats that of the model trained on MultiNLI by a huge margin on all the datasets. We attribute this difference in performance to the length of the premises present in the converted dataset, which allows the model to learn entailment relations from a long premise, unlike the much shorter premise lengths in existing NLI datasets such as MultiNLI.\comment{adding only RACE here for brevity, can include others based on whate we decide to keep in the transfer results table} \\ }

%{\sout{We want to test the effectiveness of training a model on an NLI dataset which has long premises by comparing its performance with a model trained on MultiNLI.  For this, we need NLI datasets which have long multi-sentence premises. Hence, we take the NLI form of the converted MCRC datasets to train multi-sentence NLI models. However, to have a fair comparison with the model trained on MultiNLI, we perform zero-shot evaluations on the NLI form of other MCRC datasets (other than the one on which the model is trained). Table~\ref{tab:results_long_premise} shows the results of such zero shot evaluations. We can clearly see that the performance of the models trained on the converted MCRC datasets beats that of the model trained on MultiNLI by a huge margin on all the datasets.We attribute this difference in performance to the length of the premise present in the converted dataset, which allows the model to learn entailment relations from a long premise, unlike the much shorter premise lengths in existing NLI datasets such as MultiNLI.\sout{We clearly observe that the average premise lengths (Table \ref{tab:premise_lengths}) correlates with the zero-shot transfer performance , validating our long premise conjecture \todo{write this more explicitly/clearly}.}}

\comment{[Now with the 3 point contribution structure and all the mentions of MCRC and CFCS as downstream tasks occurring together, I feel that 7.2 and 7.3 should be clubbed.]}

To validate our long premise conjecture, we analyse and contrast the zero-shot evaluation performance of models trained on the hybrid converted datasets and MultiNLI in the context of the MCRC task using the transferable modeling setup described in Section \ref{sec:transferable_modeling}. 
The results of these evaluations are presented in Table \ref{tab:results_long_premise}.  \newlyadded{We show that, in most cases, the models trained on the hybrid conversions outperforms the MultiNLI model on all \textit{other} MCRC datasets.} We assert that this difference in performance can be attributed to the difference in premise lengths of the converted datasets and MultiNLI. 
%To further substantiate this point, we highlight a high-level trend observable in Table \ref{tab:results_long_premise}. We see that as the average premise length increases (from MNLI to RACE), the zero-shot transfer performance of models trained on the respective dataset improves.}


\begin{table}[]
    \centering
    \resizebox{0.5\textwidth}{!}{%
    \begin{threeparttable}
    \begin{tabular}{l|c|c|c|c}
    \toprule
        \multirow{2}{*}{\diagbox[]{Model}{Dataset\tnote{\dag}}}
            & RACE
            & MultiRC
            & DREAM
            & CosmosQA\\
            & (271)
            & (252)
            & (110)
            & (75)\\
    \midrule
        Random Guess
            & 25.00
            & 50.00
            & 33.33
            & 33.33\\
       % Removing QA baseline because we do not want to distract with Q+A result when comparing to MultiNLI
       % Q+A RoBERTa Baselines
       %    & 84.33
       %    & 85.19
       %    & 84.22
       %    & 85.58\\
    \midrule
        MultiNLI
            & 44.34
            & 60.58
            & 67.76
            & 38.11\\
        % RACE\textsubscript{Neural}
        %     & \textit{82.89}
        %     & 77.02
        %     & 82.21
        %     & 72.56\\
        RACE\textsubscript{Hybrid}
            & \sout{\textit{83.99}}\tnote{x}
            & \textbf{77.43}
            & \textbf{83.58}
            & \textbf{73.58}\\
        % MultiRC\textsubscript{Neural}
        %     & 61.45
        %     & \textit{80.60}
        %     & 67.81
        %     & 46.96\\
        MultiRC\textsubscript{Hybrid}
            & 58.02
            & \sout{\textit{81.22}}\tnote{x}
            & 67.12
            & 43.65\\
        % DREAM\textsubscript{Neural}
        %     & 63.82
        %     & 70.35
        %     & \textit{82.41}
        %     & 56.16\\
        DREAM\textsubscript{Hybrid}
            & \textbf{65.01}
            & 71.08
            & \sout{\textit{83.99}}\tnote{x}
            & 61.00\\
        % CosmosQA\textsubscript{Neural}
        %     & 49.27
        %     & 54.72
        %     & 72.93
        %     & \textit{83.34}\\
        CosmosQA\textsubscript{Hybrid}
            & 49.27
            & 48.80
            & 72.46
            & \sout{\textit{83.89}}\tnote{x}\\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}[flushleft]
    \footnotesize
    \item [\dag] Datasets are in NLI form created using hybrid conversion method (Section \ref{subsec:conversion_hybrid}) for the hybrid models and neural conversion method (Section \ref{subsec:conversion_neural}) for the neural models and MultiNLI \comment{multili feels like it's just hanging}. 
    \item [x] These numbers are not presented as they are not the result of zero-shot evaluation. \newlyadded{Refer Table \ref{tab:all-results} for them.}
    \end{tablenotes}
    \caption{Zero-shot evaluation accuracies achieved by models trained on converted NLI datasets and MultiNLI on other MCRC datasets (in NLI form). The numbers in the parenthesis of the column headers denote the average premise lengths of the datasets.}
    \label{tab:results_long_premise}
    \end{threeparttable}
    }%
\end{table}


To present further evidence in support of our claim, 
%In order to investigate our claim further
we analyse the performance of the models trained on the hybrid conversion of RACE (RACE\textsubscript{Hybrid})
%\footnote{Our further experiments focus on RACE_\textsubscript{Hybrid} because of its consistent performance on all other MCRC datasets (Table~\ref{tab:results_long_premise}).}
and MultiNLI, with varying premise length. For the purpose of this experiment, we combine all the MCRC dev datasets described in Section \ref{sec:conversion} into a single large corpus and plot the performance with respect to the number of words in the premise in buckets of size 50. Figure \ref{fig:long_premise_conjecture} shows the sharp decline in the performance of the MultiNLI model as the length of the premise increases beyond 150 words, where as the RACE\textsubscript{Hybrid} is much more robust to increase in premise length.

% To present further evidence in support of our claim, 
% %In order to investigate our claim further
% we \sout{observe}analyse the performance of the models trained on the \sout{neural}hybrid conversion of RACE (RACE\textsubscript{Hybrid}) and MultiNLI, with \sout{respect to the}varying premise length. For the purpose of this experiment, we combine all the MCRC dev datasets described in Section \ref{subsec:diverse_qa_datasets} into a single large corpus and plot the performance with respect to the number of words in the premise in buckets of size 50. Figure \ref{fig:long_premise_conjecture} shows the sharp decline in the performance of the MNLI model as the length of the premise increases beyond 150 words, where as the RACE\textsubscript{Hybrid} is much more robust to increase in premise length.
% }
% \sout{Figure \ref{fig:long_premise_conjecture} shows the performance of these models on a combined evaluation set of all the MCRC datasets mentioned in Section \ref{subsec:diverse_qa_datasets}. From Figure \ref{fig:long_premise_conjecture}, we can clearly see that there is a} 

In the following section we further strengthen our claim by evaluating the models on another long-premise downstream task - CFCS. \comment{does it sound like we did CFCS as an afterthought? If yes, we need to change this bridge}

\sout{performs consistently well}. \sout{\comment{Not describing what the evaluation set is here because the caption does a good job of it. Hence focusing on the discussion here. These results highlight the inability of sentence-level NLI models to perform multi-sentence reasoning and validates our long-premise conjecture.}}

\sout{The graphs clearly show a sharp decline \newlyadded{(about $25\%$ on MCRC and $40\%$ on CFCS)} in MultiNLI accuracy as the premise length grows closer to 500 words. The model trained on RACE\textsubscript{Neural} also loses a bit of accuracy \newlyadded{(about $5\%$ on both MCRC and CFCS)} as the premise length grows but is far more robust than the MultiNLI model.}


\begin{figure}
    \centering
    \hspace{-10pt}\includegraphics[width=0.5\textwidth]{images/premise_len_exp_mcrc_hybrid.png}
    %\includegraphics[width=\columnwidth]{images/premise_len_exp_cfcs.png}
    \caption{The graphs show the performance of models trained on RACE\textsubscript{Hyrbid} and MultiNLI at different premise lengths on a combined evaluation set of all the MCRC datasets mentioned in Section \ref{sec:diverse_qa_datasets}.
    . 
    The accuracy at length {\em x} denotes the accuracy of the models on the examples with premise length in $[x, x+50)$ words.}
    \label{fig:long_premise_conjecture}
\end{figure}



%We compare the performance of the RoBERTa model fine-tuned on the neural converted RACE dataset with the one fine-tuned on MultiNLI \comment{(two class version)}. We show that not only does our converted dataset help RoBERTa perform better than MultiNLI,but the RoBERTa model fine-tuned on neural converted RACE dataset achieves new state-of-the-art results on all these tasks.



%\begin{table}[]
%\centering
%\begin{tabular}{@{}lccc@{}}
%\toprule
%\multirow{2}{*}{Dataset}  
%    & \multicolumn{3}{c}{Number of examples} \\\cmidrule(l){2-4} 
%        & train
%        & dev
%        & test      \\\bottomrule
%    RACE
%        & 87866
%        & 4887
%        & 4887\\
%    %RACE-subset
%        %& 48890
%        %& 2496
%        %& 2473\\
%    MultiRC
%        & 27243
%        & 4848
%        & -\\
%%MultiRC-subset & 25372        & 4458                   \\
%    DREAM
%        & 6116
%        & 2040
%        & 2041\\
%%DREAM-subset   & 5867         & 1959                   \\
%    CosmosQA
%        & 23766
%        & 2724
%        & -\\
%    BoolQ
%        & 9427
%        & 3270
%        & -\\ \bottomrule
%\end{tabular}
%\caption{Number of examples in each dataset and the corresponding subsets.\todo{\sout{Add test set stats.} We can move this table to appendix if we have space crunch and want to include something more essential.}}
%\label{tab:datasets}
%\end{table}

==> discards/related_work.tex <==
NLI has gained significant popularity due to the availability of large scale datasets~\cite{bowman2015large,williams2017broad} that can be used to train data-hungry deep learning models~\cite{kapanipathi2019infusing,wang2015learning}, including transformer-based architectures~\cite{devlin2018bert}. 

% Works relevant to the end use of these NLI models for downstream tasks has been very limited and can be categorized into: (1) Addressing the need for task-specific NLI datasets~\cite{kryscinski2019evaluating,Demszky2018}; (2) Hybrid models that are trained on native NLI dataset and its originial task (QA/Text-Summarization)~\cite{falke2019ranking,Trivedi2019}. In this section we discuss the above two categories of work.
Recent efforts to apply well-trained\comment{[Suggestion: replace well-trained with trained]} NLI models on downstream NLP tasks such as QA and CFCS have had limited success. These works have focused largely on leveraging NLI models trained on sentence-level NLI datasets. \citet{khot2018scitail} attempt to transfer knowledge between a specially curated science NLI dataset - SciTail to a QA dataset in the same domain - ARC, but their NLI model does not perform much better than the random baseline \comment{[I think you meant to site the ARC paper here Khot et. al. is SciTail creation paper. If we want to cite Khot. et. al., it should be alongside Demsky paper talking about how they \emph{manually} convert a QA dataset SciQ to an NLI dataset Scitail and talk about how that Scitail dataset has not helped with ARC while our conversion does help other MCRC datasets without fine-tuning. ]}. Similarly, \citet{kryscinski2019evaluating} show that BERT trained on MNLI is unable to do any better than the random baseline on the task of CFCS. \comment{[Suggestion: Do not mention Kryscinski paper here, let it be the third para of related work where we talk about the datasets because their main contribution is their automatically created training dataset. Combined with the comment above, I think this para should directly start with Trivedi et.al., followed by Falke et.al. and end with "divide and conquer does not work". Like one of the initial versions of related work was doing. ]}

Acknowledging the shift in premise length\comment{[Dropping in the premise length here sounds weird. We should describe the works first and then point out that they use divide and conquer.]} between NLI and downstream tasks, some works have tried to use the sentence-level NLI models by segmenting the long premise. \citet{Trivedi2019} use simple rules to first cast the problem of MCRC to NLI and subsequently divide the long passage into smaller sentence-level premises. They use a pretrained NLI model to obtain sentence-level relevance scores w.r.t a particular hypothesis 
%\sout{followed by a multi-level representation aggregation}
which is then aggregated to obtain the final score for that hypothesis.
%\sout{(answer option)}. 
\citet{falke2019ranking} apply a similar approach for the task of CFCS and divide both the provided summary as well as the source documents into single-sentence premises and hypotheses. They use a simple entailment score aggregation over all sentence-level premise-hypothesis pairs to obtain the factual correctness score for each provided summary. They show that despite this setup, out-of-the-box NLI
models do not transfer well to the task of checking factual correctness. We argue that this \emph{divide and conquer} approach is not ideal for the problem and highlight the need for a \emph{native} multi-sentence inference model.

\comment{A point I noticed is that we keep citing trivedi et. al. but we do not compare with them as a baseline (they also used MultiNLI in some form). For this, we should highlight that they do not attempt to use NLI models out-of-the-box but fine-tune to learn the aggregation.}

An interesting alternate approach to the problem has been to identify resource-rich tasks which can be easily recasted to NLI to form long premise NLI datasets. \citet{kryscinski2019evaluating} create an automatically generated training dataset for CFCS. Even though this data has long premises, the analysis done by \citet{FactCCAnalysis} finds that a model trained on this data only works for easy examples\comment{[Should we say what we mean by easy?]}.
\citet{Demszky2018} attempt to create NLI datasets that require inter-sentence reasoning by converting subsets of various QA datasets to NLI. They try two approaches for the conversion -- a rule-based and a neural model. Their neural approach uses a trained seq2seq BiLSTM-with-copy model ~\cite{gu2016copy} to convert each ``question + answer option'' into a hypothesis sentence (the corresponding passage being the premise). However, they do not show the utility of these converted datasets by training an NLI model on them. This makes it unclear whether the NLI datasets generated by the conversion is useful for any downstream task. We posit that this direction of research is promising and largely unexplored and hence, we \comment{add something short here}. We attempt to leverage to broad spectrum of datasets available for the easily convertible task of MCRC to form useful NLI datasets which can tackle the long premise tasks of MCRC as well as CFCS.

==> discards/tables.tex <==
% \begin{table}[!ht]
% \centering
% \begin{threeparttable}
% \begin{tabular}{@{}ll@{}}
% \toprule
%     \multicolumn{2}{c}{\textbf{Sentence-pair ranking task}} \\ 
%     \midrule
%         \textbf{Model}
%         & \textbf{\% Corr. ($\uparrow$)} \\ 
%     \midrule
%         BERT+MultiNLI \tnote{*} 
%             & 64.10\% \\
%         FactCC\tnote{\textdagger}
%             & 70.00\% \\
%         QAGS\tnote{\ddag}
%             & 72.10\% \\
%         RoBERTa 
%             & 56.03\% \\
%         RoBERTa+MultiNLI 
%             & 81.76\% \\
%         % RoBERTa+RACE\textsubscript{Neural} 
%         %     & \textbf{86.59\%} \\
%         \newlyadded{RoBERTa+CosmosQA\textsubscript{Hybrid}}
%             & 76.41\% \\ 
%         \newlyadded{RoBERTa+DREAM\textsubscript{Hybrid}}
%             & 78.28\% \\ 
%         \newlyadded{RoBERTa+MultiRC\textsubscript{Hybrid}}
%             & 72.21\% \\ 
%         RoBERTa+RACE\textsubscript{Hybrid} 
%             & \textbf{86.59\%} \\ 
% \midrule
%     \multicolumn{2}{c}{\textbf{Summary re-ranking task}\sout{\tnote{\mp}}}                         \\ 
%     \midrule
%         \textbf{Model}
%             & \textbf{\% Corr. ($\uparrow$)} \\
%         \midrule
%         Original/unranked
%             & 57.90\% \\
%         ESIM*
%             & 60.70\% \\
%         RoBERTa 
%             & 50.47\% \\
%         RoBERTa+MultiNLI 
%             & 49.53\% \\
%         % RoBERTa+RACE\textsubscript{Neural} 
%         %     & 73.83\% \\
%         \newlyadded{RoBERTa+CosmosQA\textsubscript{Hybrid}}
%             & 49.53\% \\ 
%         \newlyadded{RoBERTa+DREAM\textsubscript{Hybrid}}
%             & 68.22\% \\ 
%         \newlyadded{RoBERTa+MultiRC\textsubscript{Hybrid}}
%             & 67.23\% \\ 
%         RoBERTa+RACE\textsubscript{Hybrid} 
%             & \textbf{75.70}\% \\
% \bottomrule
% \end{tabular}%
% \begin{tablenotes}[flushleft]
% \footnotesize
%     %\item [\mp] Uses the validation dataset as the test dataset is not available
%     \item [*] Taken from~\citet{Falke2019}
%     \item [\textdagger] Taken from~\citet{kryscinski2019evaluating}
%     \item [\ddag] Taken from~\citet{wang2020asking}
% \end{tablenotes}
% \vspace{-5pt}
% \caption{Fraction of examples where a factually correct summary takes the first rank. RACE\textsubscript{Hybrid} refers to the converted RACE datasets.}
% \label{tab:results-summary_ranking}
% \end{threeparttable}
% \end{table}

% \begin{table}[]
% \centering
% %\resizebox{0.49\textwidth}{!}{%
% \begin{tabular}{
%     % @{}
%     l|
%     l|
%     % c|
%     c}
% \toprule
%     \textbf{Task} 
%     & \textbf{Dataset} 
%     & \textbf{
%         \begin{tabular}
%             [c]{@{}c@{}}
%             Avg Premise \\ Length
%         \end{tabular}
%         }
%     %  & \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ set size\end{tabular}} 
%     \\ 
% \midrule
%     \multicolumn{1}{l|}{\multirow{2}{*}{NLI}}  
%         & \multicolumn{1}{l|}{MultiNLI} 
%             & 22 (1.1)
%         \\ 
%     \multicolumn{1}{l|}{}  
%         & \multicolumn{1}{l|}{SNLI}     
%             & 14 (1.0)
%         \\ 
% \midrule
%     \multicolumn{1}{l|}{\multirow{5}{*}{MCRC}} 
%         & \multicolumn{1}{l|}{RACE}
%             & 271 (18.5)
%         \\
%     \multicolumn{1}{l|}{}
%         & \multicolumn{1}{l|}{MultiRC}  
%             & 252 (14.3)
%         \\
%     \multicolumn{1}{l|}{}
%         & \multicolumn{1}{l|}{DREAM}
%             & 110 (13.9)
%         \\
%     \multicolumn{1}{l|}{}
%         & \multicolumn{1}{l|}{CosmosQA} 
%             & 75 (3.8)
%         \\
%     %\multicolumn{1}{l|}{}
%     %    & \multicolumn{1}{l|}{BoolQ}
%     %        & 108 
%     %        & 14  
%     %    \\ 
% \midrule
%     \multicolumn{1}{l|}{\multirow{2}{*}{CFCS}} 
%         & \multicolumn{1}{l|}{FactCC}
%             & 546 (28.5)
%       % \\
%     %\multicolumn{1}{l|}{}
%         %& Sentence Ranking
%             %& 25 
%              %& 1000
%         \\ 
%     \multicolumn{1}{l|}{}
%         & Summary Reranking
%             & 738 (29.5)
%         \\ 
% \bottomrule
% \end{tabular}%
% %}
% \caption{The average premise length in various datasets. The numbers denote the average word count and the numbers in parenthesis denote the average sentence count. The key point to notice here is the sharp increase in premise lengths from NLI datasets to MCRC and CFCS datasets.}
% \label{tab:premise_lengths}
% \end{table}

==> extra_info/tables.tex <==
%%%% datasets
\begin{table}[]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
\multirow{2}{*}{Dataset}  & \multicolumn{2}{c}{Number of examples} \\\cmidrule(l){2-3} 
               & train        & dev         \\\bottomrule
RACE           & 87866        & 4887                   \\
RACE-subset    & 48890        & 2496                   \\
MultiRC        & 27243        & 4848                   \\
%MultiRC-subset & 25372        & 4458                   \\
DREAM          & 6116         & 2040                   \\
%DREAM-subset   & 5867         & 1959                   \\
BoolQ          & 9427         & 3270                   \\ \bottomrule
\end{tabular}
\caption{Number of examples in each dataset and the corresponding subsets.\todo{Add test set stats. We can move this table to appendix if we have space crunch and want to include something more essential.}}
\label{tab:datasets}
\end{table}

%%%%%%%%%%%%% result qa
\begin{table*}[!ht]
\centering
\begin{threeparttable}
\begin{tabular}{@{}lllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{Dataset Format (conversion method)}          \\ \cmidrule(l){2-5} 
                         & QA (None) & NLI (Rule-based) & NLI (Neural)      & NLI (Hybrid) \\ \toprule
RACE                     & \newlyadded{\textbf{84.33}}  & -                & \newlyadded{82.89} & 84.41 (running)     \\
RACE-subset              & \newlyadded{\textbf{82.00}}   & \newlyadded{80.79}         & 78.20 (update)           & 80.88 (update)      \\
DREAM                    & \newlyadded{80.74}   & -                & \newlyadded{82.41}           & \textbf{85.00}          \\
%DREAM-subset             & 79.22  & 82.79          & 84.68           & \textbf{84.99}      \\\midrule
MultiRC \tnote{*}                 & \textbf{85.19}   & -                & 80.6           & 81.22      \\
CosmosQA           & \textbf{85.78}   & -          & 83.65           & 83.94      \\
BoolQ \tnote{*}                   & 85.11   & -                & \textbf{85.84}           & -            \\ \bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize
    \item [*] Dev set numbers
\end{tablenotes}
\caption{Accuracy on the \comment{test} set of the model on different QA datasets when presented in different formats.}
\label{tab:all-results}

\end{threeparttable}
\end{table*}



%%%%%%%%%% static passage

\begin{table*}[!ht]
\centering
\begin{tabular}{@{}lllllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Random} & \multirow{2}{*}{Majority} & \multicolumn{4}{c}{Dataset Format (conversion method)}          \\ \cmidrule(l){4-7} 
                     &&& QA (None) & NLI (Rule-based) & NLI (Neural)      & NLI (Hybrid) \\ \toprule
RACE                    & 25.00 & 26.6 & 42.48& -& 43.01 & 42.95 \\
RACE-subset             & 25.00 & 27.2 & 45.50 & 45.90 & 44.23 & 45.20 \\
DREAM                   & 33.33 & 34.40 & 37.75 & -& 37.90&38.48\\
%DREAM-subset            & 33.33 & 34.20 & 37.04 &37.77 & 38.38 & 38.08 \\\midrule
MultiRC                 & 50.00 & 57.19 & \textbf{62.21} & -& 58.31 & 57.34\\
%MultiRC-subset          & 50.00 & 57.46& \textbf{64.19} & 59.6 & 57.80 & 58.00 \\
 \bottomrule
\end{tabular}
\caption{Accuracy numbers on the static-passage dev set with premise replaced with static text of equal length.}
\label{tab:static-passage-results}
\end{table*}


%%%%%%%%% MULTIRC categories

\begin{table}[]
\centering
\begin{tabular}{@{}llc@{}}
\toprule
\textbf{Question Type}    & \multicolumn{2}{c}{\textbf{Model (conv. method )}} \\ \cmidrule{2-3}
                 & \textbf{QA}      & \textbf{NLI (Neural)}   \\ \midrule
what             & \textbf{85.49}   & 80.57                   \\ \midrule
who              & \textbf{88.73}   & 83.31                   \\ \midrule
how              & \textbf{78.89}   & 74.05                   \\ \midrule
why              & \textbf{83.59}   & 83.2                    \\ \midrule
assertion        & \textbf{80.0}    & 71.48                   \\ \midrule
which            & \textbf{74.13}   & 70.69                   \\ \midrule
double questions & \textbf{85.58}   & 81.39                   \\ \midrule
when             & \textbf{83.33}   & 82                      \\ \midrule
where            & \textbf{85.91}   & 78.17                   \\ \toprule
Overall          & \textbf{84.34}   & 79.64                   \\ \bottomrule
\end{tabular}
\caption{Accuracies of QA and Neural models on heuristically determined question types in MultiRC. \todo{(The overall does not match with Table 2. Also, papers using MultiRC unusually report $\textrm{F1}_\alpha$ and $\textrm{F1}_m$)}}
\label{tab:heuristic_categories_perf_multirc}
\end{table}



%%%%%% FactCC
\begin{table}[!ht]
\centering
\begin{threeparttable}

\begin{tabular}{@{}l|c|c@{}}
\toprule
\textbf{Model}                     & \begin{tabular}[c]{@{}c@{}}\textbf{Balanced}\\ \textbf{Accuracy }\end{tabular} & \textbf{F1-score} \\ \midrule
BERT+MNLI\tnote{\textasteriskcentered}   & 51.51 & 0.0882         \\
FactCC\tnote{\textasteriskcentered}      & 74.15 & 0.5106         \\
FactCCX\tnote{\textasteriskcentered}     & 72.88 & 0.5005         \\
RoBERTa+MNLI & 50    & \todo{} \\
RoBERTa+RACE\textsubscript{Neural} & \textbf{87.58}                                                                 & \textbf{0.8657}   \\ \bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
    \footnotesize
    \item [\textasteriskcentered] Taken from~\citet{kryscinski2019evaluating}
\end{tablenotes}
\caption{Balanced accuracy on FactCC dataset.  RACE\textsubscript{Neural} refers to the converted RACE dataset created using the BART model.}
\label{tab:results-factcc}
\end{threeparttable}
\end{table}


%%%%% Ranking 
\begin{table}[!ht]
\centering
\begin{threeparttable}
\begin{tabular}{@{}lll@{}}
\toprule
\multicolumn{1}{l|}{Set}                   & \multicolumn{2}{c}{\textbf{Sentence-pair ranking task}}                    \\ \midrule
                                           & \textbf{Model}                     & \textbf{\% Corr. ($\uparrow$)} \\ \midrule
\multicolumn{1}{l|}{\multirow{5}{*}{Test}} & BERT+MNLI \tnote{*}                         & 64.1\%                         \\
\multicolumn{1}{l|}{}                      & FactCC\tnote{\textdagger}                            & 70.0\%                         \\
\multicolumn{1}{l|}{}                      & QAGS\tnote{\ddag}                              & 72.1\%                         \\
\multicolumn{1}{l|}{}                      & RoBERTa+MNLI                       & 81.76\%                        \\
\multicolumn{1}{l|}{}                      & RoBERTa+RACE\textsubscript{Neural} & \textbf{86.59\%}               \\ \bottomrule
                                           & \multicolumn{2}{c}{\textbf{Summary ranking task}}                          \\ \midrule
                                           & \textbf{Model}                     & \textbf{\% Corr. ($\uparrow$)} \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{Val}}  & Original/unranked                          & 57.9\%                         \\
\multicolumn{1}{l|}{}                      & ESIM*                              & 60.7\%                         \\
\multicolumn{1}{l|}{}                      & RoBERTa+MNLI                       & 77.12\%                        \\
\multicolumn{1}{l|}{}                      & RoBERTa+RACE\textsubscript{Neural} & \textbf{92.25\%}               \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{Test}} & Original/unranked                          & 74\%                           \\
\multicolumn{1}{l|}{}                      & ESIM\tnote{*}                              & 71\%                           \\
\multicolumn{1}{l|}{}                      & RoBERTa+MNLI                       & 75\%                           \\
\multicolumn{1}{l|}{}                      & RoBERTa+RACE\textsubscript{Neural} & \textbf{91.66\%}               \\ \bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize
    \item [*] Taken from~\citet{Falke2019}
    \item [\textdagger] Taken from~\citet{kryscinski2019evaluating}
    \item [\ddag] Taken from~\citet{wang2020asking}
\end{tablenotes}
\vspace{-5pt}
\caption{Fraction of examples where a factually correct summary takes the first rank.}
\label{tab:results-summary_ranking}
\end{threeparttable}
\end{table}


%%%%%%%% Frags

\begin{table}[]
\centering
% \resizebox{0.48\textwidth}{!}{%
\begin{tabular}{
    l|
    % c|
    c|
    c}
\toprule
% \textbf{\begin{tabular}[c]{@{}l@{}}\textbf{Semantic}\\  \textbf{Fragment}\end{tabular}} 
    \textbf{Semantic Fragment}
    % & \textbf{RACE-QA} 
    & \textbf{RACE\textsubscript{Neural}} 
    & \textbf{MNLI} \\ %\midrule
\midrule
Boolean
    % & \multicolumn{1}{c}{75.5} 
    & 86.5
    & \textbf{93.0} \\ %\midrule
Comparative
    % & \multicolumn{1}{c}{55.8} 
    & 62.2
    & \textbf{74.5} \\ %\midrule
Conditional
    % & \multicolumn{1}{c}{\textbf{83.4}} 
    & \textbf{83.4}
    & 61.1 \\ %\midrule
Counting
    % & \multicolumn{1}{c}{54.3} 
    & \textbf{62.3}
    & 54.0 \\ %\midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Monotonicity\\ (Hard)\end{tabular}} 
Monotonicity (Hard)
    % & \multicolumn{1}{c}{44.2} 
    & 50.7
    & \textbf{62.8} \\ %\midrule
% \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Monotonicity \\ (Simple)\end{tabular}}
Monotonicity (Simple)
    % & \multicolumn{1}{c}{61.8} 
    & \textbf{67.6}
    & 62.0 \\ %\midrule
Negation
    % & \multicolumn{1}{c}{70.7} 
    & \textbf{89.6}
    & 82.5 \\ %\midrule
Quantifier
    % & \multicolumn{1}{c}{56.0} 
    & 75.7
    & \textbf{77.6} \\ \midrule
\textbf{Overall}
    % & \multicolumn{1}{c}{62.7} 
    & \textbf{72.2}
    & 70.9 \\ \bottomrule
\end{tabular}%
% }
\caption{Results on the Semantic Fragments dataset from \cite{richardson2019probing}. RACE\textsubscript{Neural} refers to the converted RACE dataset created using the BART model.\comment{\textbf{Open for Comment:} Reporting only Neural and MNLI results since that's our main intended comparison.}}
\label{tab:utility_nli-semantic_fragments}
\end{table}




%%%%%%%% DNC

\begin{table}[!ht]
    \centering
    \begin{tabular}{
        l|
        % c|
        % c|
        c|
        c}
    \toprule
        \textbf{Sem. Phenomenon} 
            % & \textbf{\% of Data} 
            % & RACE-QA 
            & \textbf{RACE\textsubscript{Neural}}
            & \textbf{MNLI} \\
    \midrule
        Factuality 
            % & 7.29\% 
            % & 61.38 
            & 61.47 
            & \textbf{67.39} \\
        NER 
            % & 63.18\% 
            % & \textbf{73.19} 
            & \textbf{69.28} 
            & 58.36 \\
        Pun 
            % & 2.94\% 
            % & 50 
            & 49.71 
            & \textbf{58.54} \\
        Sentiment 
            % & 1.01\% 
            % & 93.83 
            & \textbf{94.17} 
            & 68.5 \\
        Lexicosyntactic (MV) 
            % & 1.98\% 
            % & 36.72 
            & 35.62 
            & \textbf{43.49} \\
        Lexicosyntactic (VN) 
            % & 0.27\% 
            % & 46.88 
            & 48.13 
            & \textbf{55} \\
        Lexicosyntactic (VC) 
            % & 23.32\% 
            % & \textbf{51.73} 
            & \textbf{50.25} 
            & 46.59 \\
    \midrule
        \textbf{Overall} 
            % & 100\% 
            % & \textbf{66.06} 
            & \textbf{63.22} 
            & 56.08 \\
    \bottomrule
    \end{tabular}
    \caption{Results on the Diverse Natural Language Inference dataset from \cite{poliak2018collecting}. RACE\textsubscript{Neural} refers to the converted RACE dataset created using the BART model. MV refers to the MegaVeridicality dataset; VN to the VerbNet dataset; VC to the VerbCorner dataset. \comment{\textbf{Open for Comment:} Reporting only Neural and MNLI results since that's our main intended comparison.}}
    \label{tab:utility_nli-dnc}
\end{table}
